To what extent can ASV systems naturally defend against spoofing attacks?

The current automatic speaker verification (ASV) task involves making binary decisions on two types of trials: target and non-target. However, emerging advancements in speech generation technology pose significant threats to the reliability of ASV systems. This study investigates whether ASV effortlessly acquires robustness against spoofing attacks (i.e., zero-shot capability) by systematically exploring diverse ASV systems and spoofing attacks, ranging from traditional to cutting-edge techniques. Through extensive analyses conducted on eight distinct ASV systems and 29 spoofing attack systems, we demonstrate that the evolution of ASV inherently incorporates defense mechanisms against spoofing attacks. Nevertheless, our findings also underscore that the advancement of spoofing attacks far outpaces that of ASV systems, hence necessitating further research on spoofing-robust ASV methodologies.

==> sections/asv_systems.tex <==
Due to space limitations, we briefly discuss the eight systems used in our analysis. 
Except for RawNet3~\cite{jung2022pushing}, all systems digest handcrafted acoustic features such as mel-spectrograms as the input feature. Refer to the references for full details.

\newpara{GMM-UBM.}
The Gaussian mixture model-universal background model (GMM-UBM) is a generative modelling technique used for speaker recognition~\cite{reynolds2000speaker} and text-dependent speaker verification task~\cite{larcher2014text,kinnunen2016utterance}. In this approach, before speaker enrolment, a GMM is trained by using a large amount of speech data from non-target speakers~\cite{reynolds2000speaker}. This process is known as the universal background model or UBM. The idea behind using GMM-UBM is to model the distribution of acoustical feature space by a mixture of Gaussians.



\newpara{i-vector.}
% i-vector~\cite{dehak2010front} was the state of the art until neural network systems were devised. 
% It digests handcrafted acoustic features such as mel-spectrograms or mel-frequency cepstral coefficients (MFCCs) as the input feature. 
\cite{dehak2010front} utilizes a total variability space that contains a speaker and channel variabilities concurrently. 
A Gaussian mixture model supervector, derived from a Gaussian mixture model universal background model that is fitted using the acoustic features, is projected into a lower latent space by using a total variability matrix.

\newpara{x-vector.}
\cite{snyder2018x} %is one of the most representative ASV systems. 
% It digests handcrafted acoustic features such as mel-spectrograms or MFCCs. 
%x-vector 
adopts time-delay neural networks with varying dilation values for frame-level modelling. 
Then a statistics pooling layer aggregates frame embeddings into a single utterance-level embedding by calculating their mean and standard deviations. 
Finally, two dense layers are adopted. %Refer to \cite{snyder2018x} for further details.

\newpara{ECAPA-TDNN.}
\cite{desplanques2020ecapa} employs Res2Net as the backbone processing block with a squeeze-excitation module for frame-level modelling. 
A few additional techniques such as multi-layer feature aggregation and summation are also adopted.
Context- and channel-dependent statistics pooling is devised for aggregating frame embeddings into the utterance-level embedding. 
Finally, a dense layer and a batch normalisation layer are adopted. %Refer to \cite{desplanques2020ecapa} for further details. 

\newpara{MFA-Conformer.}
\cite{zhang2022mfa} employs convolutional neural network (CNN) sub-sampling layers followed by Conformer encoder layers for the frame embedding modelling. An attentive statistics pooling layer combines frame embeddings into an utterance embedding, where frame embeddings from all encoder layers outputs are concatenated and normalized using layer normalization~\cite{ba2016layer}.\footnote{In our implementation, we adopt the context- and channel-dependent statistics pooling from ECAPA-TDNN.} Finally, a batch normalization layer and a fully-connected layer are adopted. %Refer to \cite{zhang2022mfa} for further details.

\newpara{SKA-TDNN.}
is an extension of the ECAPA-TDNN and devised a new backbone frame embedding processing mechanism (``msSKA block'' in \cite{mun2023frequency}) as well as a module that comes right after the acoustic feature (``fcwSKA block'' in \cite{mun2023frequency}) using the selective kernel attention mechanism~\cite{li2019selective}. Context- and channel-dependent statistics pooling layer aggregates frame embeddings into an utterance embedding followed by batch normalization, fully-connected, and batch normalization layers. %Full details are available in \cite{mun2023frequency}. 

\newpara{RawNet3.}
\cite{jung2022pushing} is a CNN-based system that directly digests raw waveforms. It uses the analytic filterbank layer~\cite{pariente2020filterbank}, an extension of the sinc-convolution layer, to replace acoustic features. The frame- and utterance-level modelling part is similar to that of ECAPA-TDNN. However, it includes several modifications to adapt the architecture towards raw waveform inputs; RawNet 3 repeatedly employs pooling layers to reduce the sequence length. Afterwards, a batch normalization layer and a fully-connected layer are leveraged. %Full details are available in \cite{jung2022pushing}.  

\newpara{WavLM-Large with ECAPA-TDNN.}
This system combines WavLM-Large, an SSL model with strong representations for several downstream tasks including ASV, with ECAPA-TDNN.
We freeze the WavLM and use its representation as a feature.
ECAPA-TDNN is trained using the WavLM representations in place of conventional acoustic features. 

==> sections/config.tex <==
\vspace{-6pt}
\newpara{GMM-UBM.}
We utilized the MSR Identity toolkit~\cite{sadjadi2013msr} to develop the GMM-UBM system.
The UBM was trained solely on genuine Countermeasure (CM) training data from ASVspoof 2019 LA, deliberately excluding any spoofed utterances. 
In the GMM training phase, we utilized mean adaptation with a relevance factor of 3 and configured the system with 2048 mixtures. 
For feature extraction, 60-dimensional mel-frequency cepstral coefficients and their delta and double delta derivatives were obtained with utterance-level cepstral mean and variance normalization.


\newpara{i-vector.}
We use the Kaldi toolkit~\cite{Kaldi-Povey2011} to train the i-vector system. Our implementation follows the original recipe with a modification: we omit the VoxCeleb2 test set from the training dataset to ensure consistency in training data.

\subsection{DNN-based systems}
For the remaining six DNN-based systems, we used publicly available pre-trained systems in ESPnet-SPK~\cite{watanabe2018espnet,jung2024espnet}.
We minimized hyper-parameter search and focused on setting the configurations as similar as possible to avoid unexpected intervention from other factors. 
Unless mentioned otherwise, the below configuration applies to all six systems.
We adopt a batch size of 512 and train the model for 40 epochs.
Models use Adam optimizer~\cite{kingma2015adam} for training. 
A cosine annealing learning rate scheduler with warm-ups and restarts schedules the learning rate where the maximum is $1e^{-3}$ and the minimum is $5e^{-6}$. 
% For DNN-based systems, in terms of training mechanics, the MFA-Conformer has longer warm-up iterations and does not include learning rate restarts. 
% The other five DNN systems have shorter warm-up iterations and include learning rate restarts. 
Musan~\cite{snyder2015musan} noise and RIR~\cite{ko2017study} augmentation is applied during training.
80-dimensional mel-spectrograms (i.e., mel-filterbank energy features) with a 25ms window and a 10ms shift size are used for the acoustic feature.
Speaker embeddings have 192 dimensions.
Training objective functions comprise AAM-softmax~\cite{deng2019arcface} with sub-centre and inter top-k losses~\cite{zhao2021speakin}.
Details on hyper-parameters and training schemes are available at \texttt{\url{https://github.com/espnet/espnet/blob/master/egs2/voxceleb/spk1/README.md}}.

\newpara{x-vector.} implementation follows the original architecture proposed in \cite{snyder2018x}. Its speaker embeddings are 512-dimensional. \textbf{MFA-Conformer.}
MFA-Conformer adopts six encoder blocks, each with 512-dimensional output and a CNN kernel size of 15. 10k warm-up steps are adopted. \textbf{WavLM-Large with ECAPA-TDNN.}
We use the weighted summation of the WavLM-Large model's layer-wise outputs. 

% \newpara{SKA-TDNN.} 
% \textbf{ECAPA-TDNN} also follows the original implementation where model scale of $8$, $1,024$ CNN filters are adopted. 
% \newpara{RawNet3.}

==> sections/intro_v2.tex <==
Automatic Speaker Verification (ASV) systems are biometric technologies designed to confirm whether a given speech sample belongs to a specified enrolled speaker. These systems typically evaluate performance through a protocol consisting of two types of trials: target trials, where the voice in the speech sample matches the enrolled speaker, and non-target trials, where it does not. As a crucial component of an authentication system, ASV must not only differentiate between these trials but also robustly defend against spoofing attacks (also known as presentation attacks)—efforts to deceive the system with artificially generated or modified voices. Yet, remarkably, the integration of such critical defences against spoofing attacks has been considered in only a fractional segment of the existing ASV system developments.

Meanwhile, the explosive advancements in Text-To-Speech synthesis (TTS) and Voice Conversion (VC) have heightened vulnerabilities to spoofing attacks. The accessibility of sophisticated TTS and VC systems has inadvertently equipped fraudsters with the means to generate speech data mimicking specific target individuals~\cite{GMA2023voice}. While only a subset of the latest deep-learning-based TTS and VC systems reached the perceptual quality of bonafide speech~\cite{shen2018natural, Yi2020, cooper21_ssw}, 
many systems, even those employing basic linear statistical models, have successfully fooled state-of-the-art ASV systems by then (e.g., the i-vector PLDA \cite{dehak2010front} and the x-vector \cite{snyder2018x} systems evaluated in ASVspoof 2015 \cite{wu2015asvspoof} and 2019 challenges \cite{wang2020asvspoof}). This escalating threat led to a decade of independent spoofing detection (or countermeasure, CM) system research~\cite{wu2015asvspoof}.\footnote{The spoofing detection system does not require an enrolled (or target, claimed) speaker. It makes a binary decision on whether the input is from humans or synthesised.} 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/29_attacks_v2.png}
    \caption{
    Average SPF Equal Error Rates (EERs) on 29 different spoofing attacks, chronologically displayed using eight automatic speaker verification (ASV) systems.
    The SPF-EER adopts spoof trials in place of conventional non-target trials, where in a spoof trial, the test utterance is a system-generated voice of the target speaker.
    Conventional EERs (equivalent to SV-EER in \cite{jung2022sasv}) of the ASV systems in the Vox1-O evaluation protocol are also reported as a reference. 
    }
    \label{fig:asv_progression_2019}
    \vspace{-15pt}
\end{figure}

Despite being a minority, few studies committed to broadening the scope of ASV systems by integrating the spoofing detection scenario.\footnote{Such ASV systems, designed to account for spoofing, are termed Spoofing-robust ASV (SASV). This integration introduces three trial types: (i) target, (ii) non-target, and (iii) spoof. Despite this expansion, SASV functions as a binary classifier, approving target trials while dismissing all others.}
Early SASV solutions devised a system by combining \emph{independently developed}  ASV and CM subsystems~\cite{ge2023can,liu2024generalizing,shim2022baseline}.
More contemporary efforts have shifted towards integrated solutions~\cite{mun2023towards,shim2020integrated}, leveraging the prowess of single neural networks to undertake the SASV task. 
This innovative approach is rooted in the proven capability of neural networks to process complex decisions across various fields and tasks, in this instance, simultaneously evaluating speaker identity and the authenticity of the input.
Despite differing methodologies, they share a common goal: to precisely validate only the legitimate target trials, effectively dismissing all others.

While ASV systems show vulnerability to various spoofing attacks, the severity of these threats is not uniform. The ASVspoof 2019 \cite{wang2020asvspoof} revealed that different attacks impact the ASV Equal Error Rate (EER) to varying extents. 
Subsequent analysis \cite{ge2023can} has uncovered numerous instances where an ASV system can reject spoofing attacks, even when their training regimes did not explicitly account for such scenarios (i.e., {\em zero-shot} in terms of data and scenario).
This finding indicates that ASV systems possess an inherent ability to reject spoof attempts, especially when the imitation of the target speaker's characteristics falls short.
This insight leads to two key questions: (1) Can future enhancements in ASV technology, focused exclusively on refining speaker discrimination as currently practised, prove robust enough to counter both present and future spoofing challenges? (2) How effectively can current ASV systems, utilising a zero-shot strategy, repel spoofing attacks, and which precise varieties of attacks are they adept at blocking?


To address the first question, we present a chronological analysis examining the correlation between advancements in ASV technology and their inherent defence against spoofing attacks. 
Our study spans a broad spectrum of ASV technologies, ranging from the Gaussian Mixture Model-Universal Background Model (GMM-UBM) developed in the pre-deep learning era to the latest Self-Supervised Learning (SSL) representation-based Enhanced Deep Speaker Embedding (ECAPA-TDNN).
Illustrated in Figure~\ref{fig:asv_progression_2019} and detailed further in Section~\ref{sec:results},  our findings reveal a clear evolution in ASV systems' natural defence mechanisms against spoofing attacks.\footnote{This observation, while somewhat expected—since improved speaker discrimination inherently complicates successful spoofing attempts—represents the first documentation of a clear evolutionary trend.} 
Notably, with conventional ASV error rates plummeting from $13.00$\% to 0.60\%, the systems' robustness to spoofing has increased fourfold, although these ASV systems were never explicitly designed to counter spoof scenarios.
This demonstrates a remarkable {\em zero-shot} capability; the ASV systems effectively countered spoofing attacks without any prior training on such scenarios or data. However, it's important to note that the current EER remains too high for practical application in real-world scenarios.

To address the second question, we conduct a parallel chronological analysis focused on the evolution of attack technologies. Our examination of 29 different TTS/VC systems reveals a consistent pattern; speech data spoofed using the latest algorithms proves significantly more adept at fooling ASV systems. This outcome reflects the continuous advancement in spoofing techniques.

Our analysis leads to two critical insights: (1) advancements in ASV are enhancing the robustness of existing spoofing attacks; (2) progress in TTS/VC is far outpacing that in ASV.
Given this dynamic, we emphasise the urgent need for the ASV community to intensify efforts in crafting SASV systems. Whether through integrating ASV and CM subsystems or by developing single neural networks, enhancing spoofing robustness is paramount. Without it, ASV systems lack the necessary robustness to serve as reliable authentication mechanisms.

==> tables/attack_progress_merged.tex <==


\begin{table*}
  \caption{\textcolor{red}{merge Table 2 and EERs} Specifications of spoofing attacks included in ASVspoof 2015 (S*) and 2019 LA corpora (A*). Attacks are sorted on basis of waveform and acoustic models. \textcolor{color_tts}{TTS} are highlighted in light gray color; otherwise, VC systems. DNN-based \textcolor{color_am_dnn}{acoustic} and \textcolor{color_wm_dnn}{waveform} models are highlighted in second and third columns, respectively. Unit-selection-based TTS systems are put at bottom because they are not parametric speech synthesis as other attacks.}
  \label{tab:attack_spec_full}
 {
  \begin{center}
  \begin{tabular}{rrrrrrrr}
  \toprule
  \multicolumn{3}{c}{Spoofing Attack} & \multicolumn{5}{c}{ASV} \\
  \cmidrule(lr){1-3}\cmidrule(lr){4-8}
  ID&Acoustic model&Waveform model&\rotatebox{60}{ECAPA-TDNN} &  \rotatebox{60}{MFA-Conformer}&  \rotatebox{60}{SKA-TDNN}&  \rotatebox{60}{RawNet3}&  \rotatebox{60}{WavLM-Large}\\
  \toprule
\cellcolor{color_vc}A18&\cellcolor{color_am_sm}i-vector + PLDA&\cellcolor{color_wm_dsp}LPC&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.40&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.15&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.91&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.24&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.81\\
\cellcolor{color_vc}S5&\cellcolor{color_am_sm}GMM&\cellcolor{color_wm_dsp}MLSA&\cellcolor[rgb]{0.92, 0.92, 0.92} 19.64&\cellcolor[rgb]{0.95, 0.95, 0.95} 13.55&\cellcolor[rgb]{0.96, 0.96, 0.96} 9.33&\cellcolor[rgb]{0.94, 0.94, 0.94} 14.90&\cellcolor[rgb]{0.98, 0.98, 0.98} 5.41\\
\cellcolor{color_vc}A19&\cellcolor{color_am_sm}GMM&\cellcolor{color_wm_dsp}spectral filtering&\cellcolor[rgb]{0.98, 0.98, 0.98} 4.84&\cellcolor[rgb]{0.99, 0.99, 0.99} 3.18&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.27&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.61&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.13\\
\midrule
\cellcolor{color_vc}S2&\cellcolor{color_am_sm}Linear reg.&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.98, 0.98, 0.98} 4.71&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.21&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.26&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.76&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.35\\
\cellcolor{color_vc}S1&\cellcolor{color_am_sm}DTW&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.03&\cellcolor[rgb]{0.96, 0.96, 0.96} 9.77&\cellcolor[rgb]{0.98, 0.98, 0.98} 6.03&\cellcolor[rgb]{0.96, 0.96, 0.96} 9.59&\cellcolor[rgb]{0.99, 0.99, 0.99} 3.33\\
\cellcolor{color_vc}S6&\cellcolor{color_am_sm}GMM + GV&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.91, 0.91, 0.91} 20.76&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.35&\cellcolor[rgb]{0.96, 0.96, 0.96} 11.14&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.69&\cellcolor[rgb]{0.98, 0.98, 0.98} 6.54\\
\cellcolor{color_vc}S7&\cellcolor{color_am_sm}GMM + GV&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.95, 0.95, 0.95} 12.37&\cellcolor[rgb]{0.97, 0.97, 0.97} 8.09&\cellcolor[rgb]{0.98, 0.98, 0.98} 6.26&\cellcolor[rgb]{0.97, 0.97, 0.97} 6.98&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.87\\
\cellcolor{color_vc}S8&\cellcolor{color_am_sm}GMM-tensor&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.97, 0.97, 0.97} 8.25&\cellcolor[rgb]{0.98, 0.98, 0.98} 4.99&\cellcolor[rgb]{0.99, 0.99, 0.99} 3.98&\cellcolor[rgb]{0.98, 0.98, 0.98} 5.95&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.14\\
\cellcolor{color_vc}S9&\cellcolor{color_am_sm}DTW + Kernel reg.&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.96, 0.96, 0.96} 10.34&\cellcolor[rgb]{0.98, 0.98, 0.98} 6.48&\cellcolor[rgb]{0.98, 0.98, 0.98} 5.14&\cellcolor[rgb]{0.98, 0.98, 0.98} 6.23&\cellcolor[rgb]{0.99, 0.99, 0.99} 4.34\\
\cellcolor{color_tts}S3&\cellcolor{color_am_sm}NLP + HMM&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.93, 0.93, 0.93} 18.07&\cellcolor[rgb]{0.95, 0.95, 0.95} 13.38&\cellcolor[rgb]{0.96, 0.96, 0.96} 11.71&\cellcolor[rgb]{0.95, 0.95, 0.95} 14.05&\cellcolor[rgb]{0.97, 0.97, 0.97} 7.33\\
\cellcolor{color_tts}S4&\cellcolor{color_am_sm}NLP + HMM&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.91, 0.91, 0.91} 21.06&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.46&\cellcolor[rgb]{0.95, 0.95, 0.95} 13.31&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.66&\cellcolor[rgb]{0.97, 0.97, 0.97} 8.88\\
\midrule
\cellcolor{color_vc}A17&\cellcolor{color_am_dnn}VAE&\cellcolor{color_wm_dsp}waveform filtering&\cellcolor[rgb]{0.99, 0.99, 0.99} 1.88&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.26&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.75&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.98&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.30\\
\cellcolor{color_tts}A13&\cellcolor{color_am_dnn}TTS + VC(DNN)&\cellcolor{color_wm_dsp}waveform filtering&\cellcolor[rgb]{0.95, 0.95, 0.95} 13.55&\cellcolor[rgb]{0.96, 0.96, 0.96} 11.19&\cellcolor[rgb]{0.97, 0.97, 0.97} 6.96&\cellcolor[rgb]{0.97, 0.97, 0.97} 7.85&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.16\\
\midrule
\cellcolor{color_tts}A09&\cellcolor{color_am_dnn}NLP + RNN&\cellcolor{color_wm_dsp}Vocaine&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.40&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.99&\cellcolor[rgb]{1.00, 1.00, 1.00} 1.20&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.93&\cellcolor[rgb]{1.00, 1.00, 1.00} 0.91\\
\cellcolor{color_tts}A14&\cellcolor{color_am_dnn}TTS + VC(DNN)&\cellcolor{color_wm_dsp}STRAIGHT&\cellcolor[rgb]{0.82, 0.82, 0.82} 35.20&\cellcolor[rgb]{0.84, 0.84, 0.84} 31.46&\cellcolor[rgb]{0.88, 0.88, 0.88} 26.53&\cellcolor[rgb]{0.90, 0.90, 0.90} 22.46&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.10\\
\cellcolor{color_tts}A07&\cellcolor{color_am_dnn}NLP + RNN-GAN&\cellcolor{color_wm_dsp}WORLD&\cellcolor[rgb]{0.82, 0.82, 0.82} 34.20&\cellcolor[rgb]{0.87, 0.87, 0.87} 26.66&\cellcolor[rgb]{0.90, 0.90, 0.90} 22.32&\cellcolor[rgb]{0.99, 0.99, 0.99} 2.19&\cellcolor[rgb]{0.94, 0.94, 0.94} 15.99\\
\cellcolor{color_tts}A11&\cellcolor{color_am_dnn}DNN(end2end)&\cellcolor{color_wm_dsp}Griffin-Lim&\cellcolor[rgb]{0.70, 0.70, 0.70} 49.68&\cellcolor[rgb]{0.74, 0.74, 0.74} 45.11&\cellcolor[rgb]{0.76, 0.76, 0.76} 43.31&\cellcolor[rgb]{0.78, 0.78, 0.78} 40.46&\cellcolor[rgb]{0.84, 0.84, 0.84} 32.55\\
\midrule
\cellcolor{color_tts}A08&\cellcolor{color_am_dnn}NLP + HMM-DNN&\cellcolor{color_wm_dnn}Dilated CNN&\cellcolor[rgb]{0.91, 0.91, 0.91} 20.72&\cellcolor[rgb]{0.94, 0.94, 0.94} 14.86&\cellcolor[rgb]{0.96, 0.96, 0.96} 9.88&\cellcolor[rgb]{0.97, 0.97, 0.97} 8.46&\cellcolor[rgb]{0.96, 0.96, 0.96} 9.92\\
\cellcolor{color_tts}A12&\cellcolor{color_am_dnn}NLP + RNN&\cellcolor{color_wm_dnn}WaveNet&\cellcolor[rgb]{0.79, 0.79, 0.79} 39.08&\cellcolor[rgb]{0.78, 0.78, 0.78} 40.02&\cellcolor[rgb]{0.83, 0.83, 0.83} 33.94&\cellcolor[rgb]{0.81, 0.81, 0.81} 36.36&\cellcolor[rgb]{0.89, 0.89, 0.89} 23.60\\
\cellcolor{color_tts}A15&\cellcolor{color_am_dnn}TTS + VC(DNN)&\cellcolor{color_wm_dnn}WaveNet&\cellcolor[rgb]{0.79, 0.79, 0.79} 38.92&\cellcolor[rgb]{0.79, 0.79, 0.79} 39.14&\cellcolor[rgb]{0.82, 0.82, 0.82} 34.78&\cellcolor[rgb]{0.81, 0.81, 0.81} 35.71&\cellcolor[rgb]{0.90, 0.90, 0.90} 23.16\\
\cellcolor{color_tts}A10&\cellcolor{color_am_dnn}DNN(end2end)&\cellcolor{color_wm_dnn}WaveRNN&\cellcolor[rgb]{0.69, 0.69, 0.69} 50.35&\cellcolor[rgb]{0.67, 0.67, 0.67} 52.17&\cellcolor[rgb]{0.72, 0.72, 0.72} 47.90&\cellcolor[rgb]{0.70, 0.70, 0.70} 49.69&\cellcolor[rgb]{0.77, 0.77, 0.77} 41.26\\
\midrule
\cellcolor{color_tts}S10&\cellcolor{color_am_sm}NLP + Unit-selection&\cellcolor{color_wm_dsp}waveform concat.&\cellcolor[rgb]{0.80, 0.80, 0.80} 38.25&\cellcolor[rgb]{0.77, 0.77, 0.77} 40.98&\cellcolor[rgb]{0.79, 0.79, 0.79} 38.85&\cellcolor[rgb]{0.80, 0.80, 0.80} 37.88&\cellcolor[rgb]{0.86, 0.86, 0.86} 29.15\\
\cellcolor{color_tts}A16&\cellcolor{color_am_sm}NLP + Unit-selection&\cellcolor{color_wm_dsp}waveform concat.&\cellcolor[rgb]{0.61, 0.61, 0.61} 58.22&\cellcolor[rgb]{0.59, 0.59, 0.59} 60.44&\cellcolor[rgb]{0.63, 0.63, 0.63} 56.25&\cellcolor[rgb]{0.97, 0.97, 0.97} 9.14&\cellcolor[rgb]{0.82, 0.82, 0.82} 34.76\\
\bottomrule
  \end{tabular}
  \end{center}
  }
\end{table*}

==> tables/progress.tex <==
\begin{table*}
  \caption{
  \textcolor{red}{Full data. Won't be included in the submission.}
  Vulnerability of ASV models. Six widely adopted ASV models are tested against conventional ASV protocol (``Base''), 13 different types of spoofing attacks (``A07'' -- ``A19''), and full set (``Full''). Performances reported in equal error rates (EER$\downarrow$, \%)}
  \label{tab:vulnerability}
  \resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccccc}
  \hline
  
  \textbf{ASV Model} & \textbf{Base} &  \textbf{A07} & \textbf{A08} & \textbf{A09} & \textbf{A10} & \textbf{A11} & \textbf{A12}& \textbf{A13} & \textbf{A14} & \textbf{A15}& \textbf{A16} & \textbf{A17} & \textbf{A18}& \textbf{A19} & \textbf{Full}\\
  \hline
  
  GMM-UBM & 2.62 & 61.17 & 55.79 & 9.81 & 62.14 & 65.68 & 45.13 & 51.77 & 70.31 & 61.70 & 65.36 & 3.01 & 8.91 & 10.07 & 47.74\\
  i-vector&\\
  x-vector\cite{snyder2018x,wang2020asvspoof} & 2.48 & 59.68 & 40.39 & 8.38 & 57.73 & 59.64 & 46.18 & 46.78 & 64.01 & 58.85 & 64.52 & 3.92 & 7.35 & 14.58 & N/R\\
  ECAPA-TDNN\cite{desplanques2020ecapa} & 1.35 & 34.20 & 20.72 & 2.40 & 50.35 & 49.68 & 39.08 & 13.55 & 35.20 & 38.92 & 58.22  & 1.88 & 2.40 & 4.84 & 30.99\\
  MFA-Conformer\cite{zhang2022mfa} & 0.68 & 26.66 & 14.86 & 0.99 & 52.17 & 45.11 & 40.02 & 11.19 & 31.46 & 39.14 & 60.44 & 1.26 & 1.15 & 3.18 & 29.29\\
  SKA-TDNN\cite{mun2023frequency} & 0.57 & 22.32 & 9.88 & 1.20 & 47.90 & 43.31 & 33.94 & 6.96 & 26.53 & 34.78 & 56.25 & 0.75 & 0.91 & 2.27 & 26.18\\
  RawNet3\cite{jung2022pushing} & 0.59 & 2.19 & 8.46 & 0.93 & 49.69 & 40.46 & 36.36 & 7.85 & 22.46 & 35.71 & 9.14 & 0.98 & 1.24 & 0.61 & 20.91\\
  WavLM-Large\cite{chen2022wavlm} & 0.39 & 15.99 & 9.92 & 0.91 & 41.26 & 32.55 & 23.60 & 2.16 & 15.10 & 23.16 & 34.76 & 0.30 & 0.81 & 1.13 & 18.62\\
  \hline
  \end{tabular}}
  \end{table*}

==> tables/progress_asvspoof2015.tex <==
\begin{table*}
  \caption{
    \textcolor{red}{Full data. Won't be included in the submission.}
    ASVspoof2015 version
    }
  \label{tab:vulnerability_asvspoof2015}
  \resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccccc}
  \hline
  \textbf{ASV Model} & \textbf{Base} &  \textbf{S01} & \textbf{S02} & \textbf{S03} & \textbf{S04} & \textbf{S05} & \textbf{S06}& \textbf{S07} & \textbf{S08} & \textbf{S09}& \textbf{S10} & \textbf{Full}\\
  \hline

  GMM-UBM & \\
  i-vector & \\
  x-vector\cite{snyder2018x,wang2020asvspoof} & \\
  ECAPA-TDNN\cite{desplanques2020ecapa} & 4.21 & 15.03 & 4.71 & 18.07 & 21.06 & 19.64 & 20.76 & 12.37 & 8.25 & 10.34 & 38.25 & 18.00\\
  MFA-Conformer\cite{zhang2022mfa} & 2.88 & 9.77 & 2.21 & 13.38 & 15.46 & 13.55 & 15.35 & 8.09 & 4.99 & 6.48 & 40.98 & 14.35\\
  SKA-TDNN\cite{mun2023frequency} & 2.18 & 6.03 & 2.26 & 11.71 & 13.31 & 9.33 & 11.14 & 6.26 & 3.98 & 5.14 & 38.85 & 12.22\\
  RawNet3\cite{jung2022pushing} & 3.37 & 9.59 & 2.76 & 14.05 & 15.66 & 14.90 & 15.69 & 6.98 & 5.95 & 6.23 & 37.88 & 14.49\\
  WavLM-Large\cite{chen2022wavlm} & 1.74 & 3.33 & 1.35 & 7.33 & 8.88 & 5.41 & 6.54 & 2.87 & 2.14 & 4.34 & 29.15 & 8.69\\
  \hline
  \end{tabular}}
  \end{table*}
